The Best of Both Worlds: Reinforcement Learning with Logarithmic Regret and Policy Switches

In this paper, we study the problem of regret minimization for episodic Reinforcement Learning (RL) both in the model-free and the model-based setting. We focus on learning with general function classes and general model classes, and we derive results that scale with the eluder dimension of these classes. In contrast to the existing body of work that mainly establishes instance-independent regret guarantees, we focus on the instance-dependent setting and show that the regret scales logarithmically with the horizon $T$, provided that there is a gap between the best and the second best action in every state. In addition, we show that such a logarithmic regret bound is realizable by algorithms with $O(\log T)$ switching cost (also known as adaptivity complexity). In other words, these algorithms rarely switch their policy during the course of their execution. Finally, we complement our results with lower bounds which show that even in the tabular setting, we cannot hope for regret guarantees lower than $o(\log T)$.

==> linear_mdp_proof_sketch.tex <==
\section{Linear MDP: Proof Sketch}


==> linear_mixture_mdp.tex <==
\section{Linear Mixture MDP: Proof Sketch}

\begin{assumption}\cite{ayoub2020model}
Every unknown transition model $P_h, h \in [H]$ belongs to a family $\PP_h, h \in [H]$ of known models that are available to the agent. The elements of $\PP$ are transition kernels that map state-action pairs to signed distributions over $\S$.
\end{assumption}

\begin{definition}[Linear Mixture Models]\cite{ayoub2020model}
We say that $\PP$ is a class of linear mixture models with component models $P_1, \ldots, P_d$ if $P_1, \ldots, P_d$ are transition kernels that map state-action pairs to signed measures and $P \in \PP$ if and only if 
\begin{align*}
    P(ds'|s,a) = \sum_{j=1}^d \theta_j P_j(ds'|s,a) 
\end{align*}
where $\theta \in \R^d$.
\end{definition}

\subsection{Algorithm Sketch}\todo{Write algorithm formally after we've verified that everything works.}

The idea of our approach is based on a modification of the algorithm in~\cite{ayoub2020model}. The idea is that for every $h \in [H], k \in [K]$ we keep track of a set of potential models $\BB_h^k$ that are consistent with the data we have received so far. We show that our update ensures that, with high probability, the true models $P_h^* \in \BB_h^k, \forall h \in [H], k \in [K]$. We first show how our update is performed.

%We first outline the approach in \cite{ayoub2020model}. 

% \begin{align*}
%     Q_{H+1}^k(\cdot, \cdot) = 0, \\
%     V_{h+1}(\cdot) = 0, \\
%     Q_h^k(\cdot,\cdot) = r_h(\cdot,\cdot) + \max_{P_h \in \BB_h^k} \langle P_h, V_{h+1}^k \rangle, \\
%     V_h^k(\cdot) = \max_{a} Q_h^k(\cdot, a)
% \end{align*}

\begin{align*}
    Q_{H+1}^k(\cdot, \cdot) = 0, \\
    V_{H+1}^k(\cdot) = 0, \\
    Q_h^k(\cdot, \cdot) = \min\{r_h^k(\cdot, \cdot) +  [\hat{P}^k_h V^k_h](\cdot, \cdot) + b_h^k(s,a), H\}, \\
    V_h^k(\cdot) = \max_{a \in \AA} Q_h^k(\cdot, a)
\end{align*}
for some $b_h^k(\cdot, \cdot)$ that we will define later.

Before we define the confidence set $\BB_h^k$, we need to define the following two quantities

\begin{align*}
    \hat{P}_h^{k+1} = \arg\min_{P \in \PP} \sum_{k'=1}^k \left(\langle P(\cdot|s_h^{k'}, a_h^{k'}), V_{h+1}^{k'}\rangle - y_h^{k'} \right)^2, y_h^{k'} = V_{h+1}^{k'}(s_{h+1}^{k'}) \\
    L^k_h(P_h, \hat{P}_h^k) = \sum_{\ell = 1}^{k-1}\left(\langle P_h(\cdot| s_h^{\ell}, a_h^{\ell}) - \hat{P}^k_h(\cdot| s_h^{\ell}, a_h^{\ell}), V_{h+1}^{\ell}(\cdot) \rangle\right)^2
\end{align*}

Now we let the set of potential models at step $h$ and round $k$ to be

\begin{align*}
    \BB_h^k(\beta_h^k) = \{ P \in \PP_h: L^k_h(P_h, \hat{P}_h) \leq \beta_h^k \}
\end{align*}

where $\beta_h^k$ is a parameter to be defined later. An equivalent way to write this set is

\begin{align*}
    \tilde{L}^k_h(P_h) = \sum_{\ell = 1}^{k-1}\left(\langle P_h(\cdot| s_h^{\ell}, a_h^{\ell}), V_{h+1}^{\ell}(\cdot) \rangle - y_h^{\ell}\right)^2 \\
    \BB_h^k(\beta_h^k) = \{ P \in \PP_h: \tilde{L}^k_h(P) \leq \tilde{\beta}_h^k \}
\end{align*}

for appropriately chosen $\tilde{\beta}_h^k$.\\

Let $\VV$ be the set all measurable functions that are bounded by $H$ \todo{this is different compared to Csaba's paper -- they only care about optimal functions}. We now define $f : \S \times \AA \times \VV \rightarrow \R$ and the following sets:

\begin{align*}
    \FF^*_h = \left\{f: \exists P_h \in \PP \text{ so that } f(s, a, V) = \int_\S P_h(s'| s,a) V(s') ds', \forall (s, a, V) \in \S \times \AA \times \VV \right\}\\
    \FF_h^k(\beta_h^k) = \left\{f: \exists P_h \in \BB_h^k(\beta_h^k) \text{ so that } f(s, a, V) = \int_\S P_h(s'| s,a) V(s') ds', \forall (s, a, V) \in \S \times \AA \times \VV \right\}
\end{align*}

For some norm $||\cdot||$ and some $\alpha > 0$ we denote by $\NN(\FF, \alpha, ||\cdot||)$ the covering number of the set. This means that we can find $\NN(\FF, \alpha, ||\cdot||)$ points in $\FF$ so that every other point in $\FF$ is within distance $\alpha$ from some of these points in the norm $||\cdot||$. We slightly abuse notation and let $\NN(\FF, \alpha) = \NN(\FF, \alpha, ||\cdot||_\infty) $. Moreover, when the parameter $\beta_h^k$ is clear from the context we will write $\FF_h^k = \FF_h^k(\beta_h^k), \BB_h^k = \BB_h^k(\beta_h^k)$. We define the width of this set to be

\begin{align*}
    w(\FF_h^k; s, a, V) = \sup_{f, f' \in \FF_h^k} \left( f(s,a,V) - f'(s,a,V)\right) = \sup_{P, P' \in \BB_k^h} \langle P(\cdot|s,a) - P'(\cdot|s,a), V(\cdot)\rangle
\end{align*}

Using the above notions, we are ready to define the bonus function at round $k$ and step $h$

\begin{align*}
    b_h^k(s,a) =  w(\FF_h^k; s, a, V_{h+1}^k), \forall s \in \S, a \in \AA
\end{align*}



We start by showing that the actual model $P^*_h \in \BB_h^k, \forall h \in [H], k \in [K]$ with high probability.\\

Let $\{(X_p, Y_p)\}_{p=1,2,\ldots}$ be a sequence of random variables, where $X_p$ takes values in some measurable set $\mathcal{X}$ and $Y_p$ takes values in $\R$. Let $\tilde{\FF}$ be a subset of the real bounded measurable functions with domain $\mathcal{X}$. Let $\{\mathbb{F}_p\}_{p=0,1,\ldots}$ be a filtration such that $X_1, Y_1, X_2, Y_2, \ldots, X_{p-1}, Y_{p-1}, X_p$ are $\mathbb{F}_{p-1}$ measurable and $\E[Y_p | \mathbb{F}_{p-1}] = f^*(X_p)$, for some $f^* \in \tilde{\FF}$. We denote by $\hat{f}_t = \arg\min_{f\in \tilde{\FF}}\left(f(X_p) - Y_p \right)^2$. We also define

\begin{align*}
    \tilde{\FF}_t(\beta) = \left\{ f \in \tilde{F}: \sum_{p=1}^t \left(f(X_p) - \hat{f}(X_p)) \right)^2 \leq \beta \right\}
\end{align*}


Then, the following holds.

\begin{lemma}\label{lem:helper lemma from prior work, concentration of LSE}\cite{russo2013eluder}\cite{ayoub2020model}
Let $\mathbb{F} = \{\mathbb{F}_p \}_{p=0,1,\ldots}$ be a filtration, $\{(X_p, Y_p)\}_p$ measurable random variables where $X_p \in \mathcal{X}, Y_p \in \R$. Let $\tilde{\FF}$ be a set of measurable functions from $\mathcal{X}$ to $\R$ and assume that $\E[Y_p| \mathbb{F}_{p-1}] = f^*(X_p)$ for some $f^* \in \tilde{\FF}$. Assume that $\{Y_p - f^*(X_p)\}_{p=1,\ldots}$ is conditionally $\sigma$-subgaussian given $\mathbb{F}_{p-1}$. Let $\hat{f}_t = \arg\min_{f\in \tilde{\FF}}\left(f(X_p) - Y_p \right)^2$ and $\tilde{\FF}_t(\beta) = \left\{ f \in \tilde{F}: \sum_{p=1}^t \left(f(X_p) - \hat{f}(X_p)) \right)^2 \leq \beta \right\}$. Then, for any $\alpha > 0$, with probability $1-\delta$, for all $t \geq 1$ it holds that $f^* \in \tilde{\FF}_t(\beta_t(\delta, \alpha))$, where

\begin{align*}
    \beta_t(\delta, \alpha) = 8\sigma^2\log(2\NN(\tilde{\FF},\alpha)/\delta) + 4t\alpha\left(C+ \sqrt{\sigma^2\log(4t(t+1)/\delta)} \right)
\end{align*}
\end{lemma}




The following corollary follows the same approach as in \cite{ayoub2020model}.
\begin{corollary}\label{cor:true model is in confidence intervals}
Let $\beta_k^h = 8\sigma^2\log(2\NN(\tilde{\FF},\alpha)/\delta) + 4t\alpha\left(C+  \sqrt{\sigma^2\log(4t(t+1)/\delta)} \right)$. Then, $P^*_h \in \BB_h^k, \forall h \in [H], k \in K$ with probability at least $1-\delta $.
\end{corollary} 

\begin{proof}
\todo{write proof with correct constant, check why H/2-subgaussian and not H**2/2}
\end{proof}

\begin{lemma}\label{lem:bound between the difference of estimate of Q and Q induced by policy}
With probability at least $1-\delta$, we have that for all $h \in [H], k \in [K], s \in \S, a \in \AA$

\begin{align*}
    Q_h^k(s,a) - Q_h^{\pi_k}(s,a) \leq \langle P^*_h(\cdot|s,a), V_{h+1}^k(\cdot) - V_{h+1}^{\pi_k}(\cdot)\rangle + 2b_h^k(s,a)
\end{align*}

Moreover, it holds that $Q_h^k(s,a) \geq Q_h^*(s,a)$.
\end{lemma}


\begin{proof}
Fix some $h \in [H], k \in [K], s \in \S, a \in \AA$. Throughout the proof we condition on the event that $P^* \in \BB_h^k$. 

We first show that $\langle \hat{P}_h^k(\cdot| s,a), V_{h+1}^k(\cdot) \rangle \leq \langle P^*_h(\cdot|s,a), V_{h+1}^k(\cdot) \rangle + b_h^k(s,a)$. Indeed, since $\hat{P}_h^k, P^*_h \in \BB_h^k$ we know that there are $\hat{f}_h^k, f^*_h \in \FF_h^k$ such that $\hat{f}_h^k(s,a,V) = \langle \hat{P}_h^k(\cdot|s, a), V \rangle, f^*(s,a,V) = \langle P_h^*(\cdot|s, a), V \rangle$, for any measurable function $V: \S \rightarrow [0, H]$. Hence, we have that
\begin{align*}
    \langle \hat{P}_h^k(\cdot| s,a), V_{h+1}^k(\cdot) \rangle - \langle P^*_h(\cdot|s,a), V_{h+1}^k(\cdot) \rangle = \hat{f}_h^k(s,a,V_{h+1}^k) - f^*(s,a,V_{h+1}^k) \leq \\
    |\hat{f}_h^k(s,a,V_{h+1}^k) - f^*(s,a,V_{h+1}^k) | \leq w(\FF_h^k; s, a, V_{h+1}^k) = b_h^k(s,a)
\end{align*}

Now we use the definition of $Q_h^k(s,a), Q_h^{\pi_k}(s,a)$ to get that

\begin{align*}
    Q^k_h(s, a) \leq r_h^k(s,a) + \langle \hat{P}_h^k(\cdot|s,a), V_{h+1}^k(\cdot) \rangle + b_h^k(s,a) \leq \\
    r_h^k(s,a) + \langle P^*_h(\cdot|s,a), V_{h+1}^k(\cdot) \rangle + 2b_h^k(s,a)\\
    Q^{\pi_k}_h(s, a) = r_h^k(s,a) + \langle P^*_h(\cdot|s,a), V_{h+1}^{\pi_k}(\cdot) \rangle 
\end{align*}

Combining these two, we get that

\begin{align*}
    Q^k_h(s, a) - Q^{\pi_k}_h(s, a) \leq \langle P^*_h(\cdot|s,a), V_{h+1}^k(\cdot) - V_{h+1}^{\pi_k}(\cdot)\rangle + 2b_h^k(s,a)
\end{align*}

which proves the first part of the result.

For the second part, notice that if $Q_h^k(s,a) = H$ then the statement holds trivially since $Q^*_h(s,a) \leq H$. So we can assume without loss of generality that $Q_h^k(s,a) = r_h^k(s,a) + \langle \hat{P}_h^k(\cdot|s,a), V_{h+1}^k(\cdot) \rangle + b_h^k(s,a)$. The Bellman optimality condition gives us that $Q^*_h(s,a) = r_h^k(s,a) + \langle P_h^*(\cdot|s,a), V_{h+1}^*(\cdot) \rangle $. Hence, we have that

\begin{align*}
    Q_h^k(s,a) - Q_h^*(s,a) = \langle \hat{P}_h^k(\cdot|s,a), V_{h+1}^k(\cdot) \rangle - \langle P_h^*(\cdot|s,a), V_{h+1}^*(\cdot) \rangle + b_h^k(s,a) =\\
    \langle \hat{P}_h^k(\cdot|s,a), V_{h+1}^k(\cdot) \rangle -\langle P^*_h(\cdot|s,a), V_{h+1}^k(\cdot) \rangle + \langle P^*_h(\cdot|s,a), V_{h+1}^k(\cdot) \rangle- \langle P_h^*(\cdot|s,a), V_{h+1}^*(\cdot) \rangle + b_h^k(s,a) = \\
    \langle \hat{P}_h^k(\cdot|s,a) - P^*_h(\cdot|s,a), V_{h+1}^k(\cdot)  \rangle + \langle P_h^*(\cdot|s,a), V_{h+1}^k(\cdot) - V_{h+1}^*(\cdot)  \rangle + b_h^k(s,a)
\end{align*}

Now from our previous discussion it follows that $b_h^k(s,a)  + \langle \hat{P}_h^k(\cdot|s,a) - P^*_h(\cdot|s,a), V_{h+1}^k(\cdot)  \rangle \geq 0$. Hence, it suffices to show that $\langle P_h^*(\cdot|s,a), V_{h+1}^k(\cdot) - V_{h+1}^*(\cdot)  \rangle \geq 0$. To do that, we can just prove that $V_{h+1}^k(s') - V_{h+1}^*(s') \geq 0, \forall s' \in \S$. Since $V_{H+1}^k(s') = V_{H+1}^*(s') = 0, \forall s' \in \S$ we get that $Q_H^k(s,a) \geq Q_H^*(s,a)$. Thus, if we combine this with the update rule for $V_h^k, V_h^*$ we get the claim by induction.
\end{proof}


We now state an important lemma from \cite{russo2013eluder, ayoub2020model} that will help us bound the bonus functions that we are using. Following their notation, we define $x_{1:t} = (x_1,\ldots,x_t) \in \mathcal{X}^t, \FF|_{x_{1:t}} = \{(f(x_1), \ldots, f(x_t)), f \in \FF \}$ which is a subset of $\R^t$ and for some $S \subseteq \R^t$ we let $\text{diam}(S) = \sup_{u,v\in S}||u-v||_2$. Notice that when $S = \R$ then $\text{diam}(S) = \sup_{u,v\in S} (u - v)$

\begin{lemma}\label{lem:helper lemma about width from prior work}\cite{russo2013eluder, ayoub2020model}
 Let $\tilde{\FF}$ a set of measurable functions from some domain $\mathcal{X}$ to $\R$ bounded by $C > 0$, $\{\tilde{\FF}_t\}_{t\geq 1}$ and $\{x_t\}_{t\geq 1}$ be sequences such that $\tilde{\FF}_t \subseteq \tilde{\FF}$ and $x_t \in \mathcal{X}, \forall t \geq 1$. Then, for any $T \geq 1, \alpha > 0$ it holds that

\begin{align*}
    \sum_{t=1}^T\text{diam}(\tilde{\FF}_t|_{x_t}) \leq \alpha + C\min\{\text{dim}_E(\FF,\alpha), T\} + 2\delta_T\sqrt{\text{dim}_E(\FF,\alpha) T}
\end{align*}

where $\delta_T = \max_{1\leq t\leq T} \text{diam}(\FF_T|_{x_{1:t}})$
\end{lemma}


We will use the previous lemma to show how we can get a bound on the summation of the bonus functions for every set of rounds.

\begin{lemma}\label{lem:linear mixture sum of bonus function is bounded}
 For any set $K' \subseteq K$ and $h \in [H], \alpha > 0$ and $\FF_h^*, \FF_h^{k'}(\beta_h^{k'})$ as defined above \todo{add labels} with probability at least $1-???2$ we have that
\begin{align*}
    \sum_{i=1}^{K'}  b_h^{k_i}(s_h^{k_i},a_h^{k_i}) \leq \alpha + H\min\{\text{dim}_E(\FF,\alpha), K'\} + 4\sqrt{\text{dim}_E(\FF,\alpha) \beta_h^{K'}K'}
\end{align*}
\todo{something that depends on H is probably missing, have to pick correct beta}
where $C > 0$ is some constant.
\end{lemma}

\begin{proof}
Throughout the proof we condition on the event that $P^*_h \in \cap \BB_h^k$. We let $\tilde{\FF} = \FF_h^*, \tilde{\FF}_t = \FF_h^{k'} (\beta_h^{k'}), \mathcal{X} = \S \times \AA \times \VV, x_t = (s_h^{k'}, a_h^{k'}, V_h^{k'+1})$. Thus, the bound $C=H$ in Lemma~\ref{lem:helper lemma about width from prior work}. Using that, we get

\begin{align*}
    \sum_{i=1}^{K'} b_h^{k_i}(s_h^{k_i}. a_h^{k_i}) = \sum_{i=1}^{K'} \sup_{f, f' \in \FF_h^{k_i}(\beta_h^{k_i})} \left(f(s_h^{k_i}, a_h^{k_i}, V_h^{k_i+1}) - f(s_h^{k_i}, a_h^{k_i}, V_h^{k_i+1}) \right)\\
    \sum_{i=1}^{K'} \text{diam}\left(\FF_h^{k_i}(\beta_h^{k_i})|_{x_{k_i}}\right) \leq \alpha + H \min\{ \text{dim}_E(\FF, \alpha), K'\} + 2 \delta_{K'}\sqrt{\text{dim}_E(\FF, \alpha) K'}
\end{align*}

where the last inequality holds by Lemma~\ref{lem:helper lemma about width from prior work}. Now it remains to bound $\delta_{K'}$. Notice that $\text{diam}(\FF_h^{k_i}(\beta_h^{k_i})|{x_{1:K'}}) \leq 2 \sqrt{\beta_h^{k_i}}$. Moreover, notice that the sequence of $\beta_h^{k_i}$ is increasing, hence we can bound this quantity by the last $k_i = K'$. This gives us the result.
\end{proof}

\todo{we have all the components now. it remains to combine them similarly as in the first model.}

\begin{lemma}\label{lem:indicator bound in each interval for linear mixture model}
For every $h \in [H]$ and $n \in \N$, with probability at least 1 - ????, we have that

\begin{align*}
    \sum_{k=1}^K \mathbbm{1}\left[V_h^*(s_h^k) - Q_h^{\pi_k}(s_h^k,a_h^k) \geq 2^n \text{gap}_{\min} \right] \leq ?????
\end{align*}
 
 \end{lemma}
 
 
 \begin{proof}
 We keep $h$ fixed. We also let $k_0 = 0$, and $k_i, i \in [N]$ to be
the minimum index of the episode where the gap is at least $2^n \text{gap}_{\min}$, i.e.
\begin{align*}
    k_i = \min\{k: k > k_{i-1}, V_h^*(s_h^k) - Q_h^{\pi_k}(s_h^k, a_h^k) \geq 2^n \text{gap}_{\min} \}
\end{align*}

We denote by $K'$ the number of episodes where the gap at step $h$ is at least $2^n$, i.e.

\begin{align*}
    K' = \sum_{k=1}^K \mathbbm{1}\left[ V^*_h(s_h^k) - Q_h^{\pi_k}(s_h^{k_i}, a_h^{k_i}) \geq 2^n \text{gap}_{\min}\right]
\end{align*}


The goal is to bound the quantity $\sum_{i=1}^{K'}\left(Q_h^{k_i}(s_h^{k_i},a_h^{k_i}) - Q_h^{\pi_{k_i}}(s_h^{k_i}, a_h^{k_i})\right)$ from below and above with functions
$f_1(K'), f_2(K')$ and then use the fact that $f_1(K') \leq f_2(K')$ to derive an upper bound on $K'$.

For the lower bound, we have that

\begin{align*}
    \sum_{i=1}^{K'}\left(Q_h^{k_i}(s_h^{k_i},a_h^{k_i}) - Q_h^{\pi_{k_i}}(s_h^{k_i}, a_h^{k_i})\right) \geq \sum_{i=1}^{K'}\left(Q_h^{k_i}(s_h^{k_i},\pi_h^*(s_h^{k_i},h)) - Q_h^{\pi_{k_i}}(s_h^{k_i}, a_h^{k_i})\right) \\
    \geq \sum_{i=1}^{K'}\left(Q_h^*(s_h^{k_i},\pi_h^*(s_h^{k_i},h)) - Q_h^{\pi_{k_i}}(s_h^{k_i}, a_h^{k_i})\right) 
    = \sum_{i=1}^{K'}\left(V_h^*(s_h^{k_i}) - Q_h^{\pi_{k_i}}(s_h^{k_i}, a_h^{k_i})\right) \geq 2^n \text{gap}_{\min} K'
\end{align*}

where the first inequality holds by the definition of the policy $p_{k_i}$, the second one follows because $Q^{k_i}_i(\cdot, \cdot)$ is an optimistic estimate of $Q^*_h(\cdot, \cdot)$ which happens with probability at least $1-\delta_1/2$ (see Lemma~\ref{lem:bound between the difference of estimate of Q and Q induced by policy}) and the second one by the definition of $k_i$.

We get the upper bound on this quantity in the following way. For any $h' \in H$ we have

\begin{align*}
    Q_{h'}^k(s_{h'}^k, a_{h'}^k) - Q_{h'}^{\pi_k}(s_{h'}^k, a_{h'}^k) \leq \sum_{s'\in \S}P_{h'}(s'|s_{h'},a_{h'})V^k_{h'+1}(s') + r_{h'}(s_{h'}, a_{h'}) + 2b_{h'}^k(s_{h'}^k, a_{h'}^k) - Q_{h'}^{\pi_k}(s_{h'}^k, a_{h'}^k) = \\
    [P_{h'}(V_{h'+1}^k - V_{h'+1}^{\pi_k})](s_{h'}^k, a_{h'}^k) + 2b_{h'}^k(s_{h'}^k, a_{h'}^k) = V_{h'+1}^k(s_{h'+1}^k) - V_{h'+1}^{\pi_k}(s_{h'+1}^k) + \epsilon_{h'}^k + 2b_{h'}^k(s_{h'}^k, a_{h'}^k) = \\
    Q_{h'+1}^k(s_{h'+1}^k, a_{h'+1}^k) - Q_{h'+1}^{\pi_k}(s_{h'+1}^k, a_{h'+1}^k) + \epsilon_{h'}^k + 2b_{h'}^k(s_{h'}^k, a_{h'}^k)
\end{align*}
where we define $\epsilon_{h'}^k = [P_{h'}(V_{h'+1}^k - V_{h'+1}^{\pi_k})](s_{h'}^k, a_{h'}^k) - (V_{h'+1}^k(s_{h'+1}^k) - V_{h'+1}^{\pi_k}(s_{h'+1}^k))$ and the inequality follows from Lemma~\ref{lem:bound between the difference of estimate of Q and Q induced by policy}.

We now take the summation over all $k \in K', h \leq h' \leq H$ and we get

\begin{align*}
    \sum_{i=1}^{K'} \left( Q_h^{k_i}(s_h^{k_i}, a_h^{k_i}) - Q_h^{\pi_{k_i}}(s_h^{k_i}, a_h^{k_i}) \right) \leq \sum_{i=1}^{K'} \sum_{h'=h}^H\epsilon_{h'}^{k_i} + \sum_{i=1}^{K'} \sum_{h'=h}^H b_{h'}^{k_i}(s_{h'}^{k_i}, a_{h'}^{k_i})
\end{align*}

We will bound each of the two terms on the RHS separately. 

For the first term, we notice that $x_j = [P_{j}(V_{j+1}^{k_i} - V_{j+1}^{\pi_{k_i}})](s_{j}^{k_i}, a_{h'}^{k_i}) - (V_{j+1}^{k_i}(s_{j+1}^{k_i}) - V_{j+1}^{\pi_{k_i}}(s_{j+1}^{k_i}))$ forms a martingale difference sequence with zero mean and $|x_j| \leq 2H$. Hence, we can use Lemma~\ref{lem:azuma-hoeffding inequality} and  that for each $k\in[K]$, with probability at least $1-\delta$ we have that

\begin{align*}
    \sum_{i=1}^k \sum_{j=1}^H \left( [P_{j}(V_{j+1}^{k_i} - V_{j+1}^{\pi_{k_i}})](s_{j}^{k_i}, a_{h'}^{k_i}) - (V_{j+1}^{k_i}(s_{j+1}^{k_i}) - V_{j+1}^{\pi_{k_i}}(s_{j+1}^{k_i})) \right) \leq \sqrt{8k H^2 \log(1/\delta)}
\end{align*}

If we take the union bound over all $k\in [K]$ we have that with probability at least $1-K'\delta$

\begin{align*}
    \sum_{i=1}^{K'} \sum_{h'=h}^H\epsilon_{h'}^{k_i} \leq \sqrt{8 K' H^2 \log(1/\delta)} 
\end{align*}

We now focus on the second term. Using Lemma~\ref{lem:linear mixture sum of bonus function is bounded} we get that

\begin{align*}
    \sum_{i=1}^{K'} \sum_{h'=h}^H b_{h'}^{k_i}(s_{h'}^{k_i}, a_{h'}^{k_i}) \leq \sum_{h'=h}^H \left(\alpha + H\min\{\text{dim}_E(\FF,\alpha), K'\} + 4\sqrt{\text{dim}_E(\FF,\alpha) \beta_h^{K'}K'} \right) \\ \leq 
    \alpha + H^2\text{dim}_E(\mathcal{F}, \alpha) + 4H\sqrt{\text{dim}_E(\mathcal{F},\alpha)\beta_h^{K'}K'} 
\end{align*}

and this happens with probability at least $1-???$. Hence, combining the upper and lower bound of $$\sum_{i=1}^{K'}\left(Q_h^{k_i}(s_h^{k_i},a_h^{k_i}) - Q_h^{\pi_{k_i}}(s_h^{k_i}, a_h^{k_i})\right)$$ we get that

\todo{for now I pick alpha = 1/HT  and the constants are crude--we will use a different algorithm anyway}
(for this choice of $\alpha$ we have roughly that $\beta_h^{K'} \leq 8H^2\log (2 \NN(\FF, 1/T)) + 4(C + 8\sqrt{H^2\log(T/\delta)})$
\begin{align*}
    2^n \text{gap}_{\min}K' \leq \sqrt{8 K' H^2 \log(1/\delta)} +\alpha + H^2\text{dim}_E(\mathcal{F}, \alpha) + 4H\sqrt{\text{dim}_E(\mathcal{F},\alpha)\beta_h^{K'}K'}  \leq \\
    \sqrt{9 K' H^2 \log(1/\delta)} + C'H^2\text{dim}_E(\FF, 1/T)\sqrt{\log (2 \NN(\FF, 1/T))K'\log(T/\delta)}  \\
     \implies K' \leq \frac{\tilde{C} H^6 \log(T/\delta) \text{dim}^2_E(\FF, 1/T) \NN(\FF,1/T)}{4^n \text{gap}_{\min}^2}
\end{align*}
 \end{proof}
 
 

\begin{lemma}\label{lem:linear mixture sum of suboptimalities over all K for some h}
For come constant C and for $h \in [H]$ we have that with probability at least $1-????$

\begin{align*}
    \sum_{k=1}^K \left( V_h^*(s_h^k) - Q_h^*(s_h^k, a_h^k) \right) \leq\frac{\tilde{C} H^6 \log(T/\delta) \text{dim}^2_E(\FF, 1/T) \NN(\FF,1/T)}{ \text{gap}_{\min}}
\end{align*}


\end{lemma}

\begin{proof}
Throughout this proof we condition on the event described in Lemma~\ref{lem:indicator bound in each interval for linear mixture model} which happens with probability at least $1-??$. Since $\text{gap}_{\min} > 0$ whenever we do not take the optimal action, we have that either $V_h^*(s_k) - Q_h^*(s_h^k, a_h^k) = 0$ or $V_h^*(s_k) - Q_h^*(s_h^k, a_h^k) \geq \text{gap}_{\min}$. Our approach is to divide the interval $[0, H]$ into $N = \lceil \log(H/\text{gap}_{\min})\rceil$ intervals and count the number of $V_h^*(s_k) - Q_h^*(s_h^k, a_h^k)$ that fall into each interval. Notice that for every $V_h^*(s_k) - Q_h^*(s_h^k, a_h^k)$ that falls into interval $i$ we can get an upper bound of $V_h^*(s_k) - Q_h^*(s_h^k, a_h^k) \leq 2^i\text{gap}_{\min}$ and this upper bound is essentially tight. Hence, we have that

\begin{align*}
    \sum_{k=1}^K \left( V_h^*(s_h^k) - Q_h^*(s_h^k, a_h^k) \right) \leq \sum_{i=1}^N \sum_{k=1}^K \mathbbm{1}\left[ 2^i\text{gap}_{\min} \geq V_h^*(s_h^k) - Q_h^*(s_h^k, a_h^k) \geq 2^{i-1}\text{gap}_{\min} \right] \cdot 2^i \text{gap}_{\min} \\
    \leq \sum_{i=1}^N \sum_{k=1}^K \mathbbm{1}\left[  V_h^*(s_h^k) - Q_h^*(s_h^k, a_h^k) \geq 2^{i-1}\text{gap}_{\min} \right] \cdot 2^i \text{gap}_{\min} \\
    \leq \sum_{i=1}^N \frac{\tilde{C} H^6 \log(T/\delta) \text{dim}^2_E(\FF, 1/T) \NN(\FF,1/T)}{4^{i-1} \text{gap}_{\min}^2} \cdot 2^i \text{gap}_{\min} \\
    = \sum_{i=1}^N \frac{C' H^6 \log(T/\delta) \text{dim}^2_E(\FF, 1/T) \NN(\FF,1/T)}{2^i \text{gap}_{\min}} \\
    \leq
    \frac{C H^6 \log(T/\delta) \text{dim}^2_E(\FF, 1/T) \NN(\FF,1/T)}{ \text{gap}_{\min}} 
\end{align*}

where the first inequality holds by the definition of the intervals, the second due to the properties of the indicator function, the third because of Lemma~\ref{lem:indicator bound in each interval for linear mixture model} and in the last two steps we just manipulate the constants. 
\end{proof}


We are now ready to state the regret bound of our algorithm.
\begin{theorem}\label{thm:regret guarantee for linear mixture MDP}
There exists a constant $C$ and proper values of the parameters of the algorithm \todo{write algorithm, parameters} such that with probability at least $1- \lceil \log T \rceil e^{-\tau} -?????$ the regret of the algorithm is bounded by

\begin{align*}
    \text{Regret}(K) \leq \frac{C H^7 \log(T/\delta) \text{dim}^2_E(\FF, 1/T) \NN(\FF,1/T)}{ \text{gap}_{\min}}  + \frac{16 H^2 \tau}{3} + 2
\end{align*}

In particular, the dependence of the regret in the time horizon $T$ is logarithmic.
\end{theorem}

\begin{proof}
Throughout the proof, we condition on the events described in Lemma~\ref{lem:regret decomposition},~\ref{lem:linear mixture sum of suboptimalities over all K for some h} which happen with probability at least $1- \lceil \log T \rceil e^{-\tau} -??????$.

From Lemma~\ref{lem:regret decomposition} we have that

\begin{align*}
    \text{Regret}(K) \leq 2 \sum_{k=1}^K\sum_{h=1}^H \text{gap}_h(s_h^k, a_h^k) + \frac{16 H^2 \tau}{3} + 2
\end{align*}

We can bound the first term on the RHS using Lemma~\ref{lem:linear mixture sum of suboptimalities over all K for some h} as follows

\begin{align*}
    2 \sum_{k=1}^K\sum_{h=1}^H \text{gap}_h(s_h^k, a_h^k) = 2 \sum_{k=1}^K\sum_{h=1}^H  \left( V_h^*(s_h^k) - Q_h^*(s_h^k, a_h^k) \right) \leq \frac{2C H^7 \log(T/\delta) \text{dim}^2_E(\FF, 1/T) \NN(\FF,1/T)}{ \text{gap}_{\min}}
\end{align*}

This gives us the result.

\end{proof}

==> linear_mixture_mdp_logarithmic_adaptivity.tex <==
\section{Linear Mixture MDP: Logarithmic Adaptivity}

The idea is to use the approach of \cite{kong2021online} and do the regression that we described in the previous section but at every time step, we perform the update with some probability. We can either keep the whole dataset or sub-sample the dataset. We follow the approach of~\cite{kong2021online}.\\

On top of the definition we were using before, we have the following:

\todo{maybe $X_h^k = (s_h^k, a_h^k, V_{h+1}^k)), Y_h^k = (V_{h+1}^k)$}

\begin{align*}
    \LL_h^k = \{\left((s_h^\tau, a_h^\tau, V_{h+1}^{\tau}(\cdot)), V_{h+1}^{\tau}(s_{h+1}^\tau, a_{h+1}^\tau)\right) \}_{\tau \in [k-1]},\\
    \ZZ_h^k = \{((s_h^\tau, a_h^\tau, V_{h+1}^{\tau}(\cdot)) \}_{\tau \in [k-1]}
x\end{align*}

We also denote by $\hat{\ZZ}_h^k$ the sub-sampled dataset. We will describe the sampling procedure later.

\begin{align*}
    \hat{P}_h^{k+1} = \arg\min_{P \in \PP} \sum_{k'=1}^k \left(\langle P(\cdot|s_h^{k'}, a_h^{k'}), V_{h+1}^{k'}\rangle - y_h^{k'} \right)^2, y_h^{k'} = V_{h+1}^{k'}(s_{h+1}^{k'}) \\
    L_{\ZZ}(P_1, P_2) = \sum_{(s,a,V)\in \ZZ }\left(\langle P_1(\cdot| s, a) - P_2(\cdot| s,a), V(\cdot) \rangle\right)^2 \\
     L_{\ZZ}(f_1, f_2) = \sum_{(s,a,V)\in \ZZ }\left( f_1(s,a,V) - f_2(s,a,V)\right)^2
\end{align*}

Now we let the set of potential models at step $h$ and round $k$ to be

\begin{align*}
    \BB_{h,\ZZ}(\hat{f}, \beta) = \{ f \in \FF_h: L_\ZZ(f, \hat{f}) \leq \beta \}
\end{align*}

%where $\beta_h^k$ is a parameter to be defined later.

We slightly abuse the notation and define the following sets for every $h \in [H], k \in [K]$:

\begin{align*}
    \underbar{$\CC$}_h^k(\alpha) = \BB_{h,\ZZ_h^k}(\hat{f}_h^k, \alpha/100)\\
    \hat{\CC}_h^k(\alpha) =
    \left\{f \in \FF_h| \min\{||f - \hat{f}_h^k||_{\hat{\ZZ}_h^k}, T(H+1)^2\} \leq \alpha\right\}\\
    %\BB_{h,\hat{\ZZ}_h^k}(\hat{P}_h^k, \alpha)\\
    \overline{\CC}_h^k(\alpha) = \BB_{h,\ZZ_h^k}(\hat{f}_h^k, 100\alpha)
\end{align*}

Our goal is to show that $\underbar{$\CC$}_h^k(\alpha) \subseteq \hat{\CC}_h^k(\alpha) \subseteq \overline{\CC}_h^k(\alpha)$ with high probability. Let $\EE_h^k(\alpha)$ denote the event that this holds. We also denote by $\EE_h^k = \cap_{n=0}^\infty \EE_h^k(100^n\beta)$\todo{I'm not sure if we need infinity. The proof they have holds for a bounded alpha and I think this should be good enough}. This is event will show us that $\hat{\ZZ}_h^k$ is a good approximation to $\ZZ_h^k$.\\

The following lemma which is inspired by~\cite{kong2021online} establishes that fact.

\begin{lemma}\label{lem: mixture mdp: sub-sampled dataset is good approximation to original one}
The probability that all the events $\EE_h^k$ happen satisfies
\begin{align*}
    \Pr\left(\bigcap_{k=1}^k \bigcap_{h=1}^H \EE_h^k \right) \geq 1 - \delta
\end{align*}
\end{lemma}

To prove Lemma~\ref{lem: mixture mdp: sub-sampled dataset is good approximation to original one} we need the following concentration inequality proved by Freedman~\cite{freedman1975tail}.

\begin{lemma}\label{lem:freedman's concetration lemma}
Let $\{Y_i\}_{i \in \N}$ be a real-valued martingale with difference sequence $\{X_i\}_{i \in \N}$. Let $R$ be a uniform bound on $X_i$. Fix some $n \in \N$ and let $\sigma^2$ be a number such that

\begin{align*}
    \sum_{i=1}^n \E[X_i^2|Y_0, \ldots, Y_{i-1}] \leq \sigma^2
\end{align*}

Then, for all $t \geq 0$ we have that

\begin{align*}
    \Pr(|Y_n - Y_0| \geq t) \leq 2\exp{\left\{ -\frac{t^2/2}{\sigma^2 + Rt/3}\right\}}
\end{align*}
\end{lemma}


The following lemma follows the approach of~\cite{kong2021online}

\begin{lemma}\label{lem:helper lemma to prove approximation of sub-sampled dataset}

For any $\alpha \in [\beta, T(H+1)^2]$ and $k \in [K]$ we have the following bound for the probability that all the events $\{\EE_h^i\}_{i\leq k-1}$ happen and the last one does not happen

\begin{align*}
    \Pr\left( \left(\bigcap_{i=1}^{k-1} \EE_h^i\right) \EE_h^k(\alpha)^c\right) \leq ??? \delta/(32 T^2)
\end{align*}

\end{lemma}


\begin{proof}
Let $C$ be the constant that multiplies the sensitivity in the sampling probability (we will use something like $C \log(T\NN(\FF,\sqrt{\delta/64 T^3})/\delta)$ as they do). We fix some $h \in [H]$ throughout the proof.

We consider a fixed pair of functions $f_h^1, f_h^2$ in the discretized set \todo{define that formally }and for $i \geq 2$ we let $$Z_i = \max\left\{||f_h^1 - f_h^2||^2_{\ZZ_h^i}, \min\{||f_h^1 - f_h^2||^2_{\hat{\ZZ}_h^{i-1}}, T(H+1)^2\}\right\}$$\todo{maybe need $i-1$ instead of $i$, will check later}

\begin{align*}
    Y_i = 
    \begin{cases}
    \frac{1}{p_{z_h^{i-1}}}(f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2 & \text{$z_h^{i-1}$ is added to $\hat{\ZZ}_h^i$ and $Z_i \leq 2000000 \alpha$}\\
    0, & \text{$z_h^{i-1}$ is not added to $\hat{\ZZ}_h^i$ and $Z_i \leq 2000000 \alpha$} \\
    (f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2 & \text{otherwise}
    \end{cases}
\end{align*}

Let $\mathbb{F}_i$ be the filtration that $Y_i$ is adapted to. Our goal is to use Freedman's inequality (i.e. Lemma~\ref{lem:freedman's concetration lemma}) for $Y_i$.
Notice that $\E[Y_i | \mathbb{F}_i] = (f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2$\todo{this is what they have in their proof but I'm not sure that it's true}. Now we focus on the variance of $Y_i$. Notice that if $p_{z_h^{i-1}} = 1$ or $Z_i > 2000000\alpha$ then $Y_i$ is deterministic $Y_i - \E[Y_i | \mathbb{F}_{i-1}] = \text{Var}[Y_i - \E[Y_i | \mathbb{F}_{i-1}]] = 0$. For the other case, recall that $p_{z_h^i} = \min\{1, C\cdot \text{sensitivity}_{\hat{\ZZ}_h^{i-1}, \FF_h}(z_h^i) \}$ and 

\begin{align*}
    \text{sensitivity}_{\ZZ, \FF}(z) = \min\left\{\sup_{f_1, f_2 \in \FF}  \frac{(f_1(z) - f_2(z))^2}{\min\{||f_1 - f_2||_{\mathcal{\ZZ}}, T(H+1)^2\}+\beta}, 1\right\}
\end{align*}

Since $p_{z_h^{i-1}} < 1 \implies \text{sensitivity}_{\hat{\ZZ}^{i-1}_h, \FF_h}(z_h^i) < 1$. Thus, we can see that 

\begin{align*}
    Y_i \geq \E[Y_i|\mathbb{F}_i] \implies |Y_i - \E[Y_i] | \leq Y_i \leq  \frac{(f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2}{p_{z_h^{i-1}}} \leq \frac{(f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2}{C_1\sup_{f_1, f_2 \in \FF_h}  \frac{(f_1(z_h^i) - f_2(z_h^i))^2}{\min\{||f_1 - f_2||_{\mathcal{\hat{\ZZ}}_h^{i-1}}, T(H+1)^2\}+\beta}} \\
    \leq \frac{(f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2 \min\{||f_1 - f_2||_{\mathcal{\hat{\ZZ}}_h^{i-1}}, T(H+1)^2\}+\beta\}}{C_1(f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2} = \\
    (\min\{||f_1 - f_2||_{\mathcal{\hat{\ZZ}}_h^{i-1}}, T(H+1)^2\}+\beta) \cdot 1/C_1 \leq
    2000001\alpha/C_1 < 3000000\alpha/C_1
\end{align*}

where the second inequality follows from the fact that $p_{z_h^{i-1}} < 1$, the third inequality follows by the definition of supremum and the fourth one by the fact that $\alpha \geq \beta$.

For the variance, we can see that

\begin{align*}
    \text{Var}[Y_i - \E[Y_i | \mathbb{F}_i]|\mathbb{F}_i] \leq
    \E[Y_i^2 | \mathbb{F}_i] = p_{z_h}^{i-1} \left( \frac{1}{p_{z_h^{i-1}}}(f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2\right)^2 + (1-p_{z_h}^{i-1})\cdot 0 =\\
     \frac{1}{p_{z_h^{i-1}}}(f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^4 \leq 3000000\alpha (f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2 /C_1
\end{align*}


where the first inequality follows from the fact that $Y_i \geq \E[Y_i|\mathbb{F}_i]$ and the second one from the inequality we derived right above. Let $k'$ be the maximum number $\leq k$ such that $Z_{k'} \leq 2000000\alpha$. Summing up the above inequalities for $i=2,\ldots,k$ we get

\begin{align*}
    \sum_{i=2}^k \text{Var}[Y_i - \E[Y_i | \mathbb{F}_i]|\mathbb{F}_i] = \sum_{i=2}^{k'} \text{Var}[Y_i - \E[Y_i | \mathbb{F}_i]|\mathbb{F}_i] \leq\\ \frac{3000000\alpha}{C_1} \sum_{i=2}^{k'}(f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2 \leq \frac{3000000\alpha \cdot 2000000\alpha}{C_1} \leq
    \frac{(3000000\alpha)^2}{C_1}
\end{align*}


where the the first equality follows from the fact that for $i > k'$ the random variable is deterministic, the first inequality follows by the summation of the previous one and the second one by the fact that $\sum_{i=2}^{k'}(f_h^1(z_h^{i-1}) - f_h^2(z_h^{i-1}))^2 \leq ||f_h^1 - f_h^2||_{\ZZ_h^{k'}} \leq Z_{k'}$.

We are now ready to use Freedman's inequality (Lemma~\ref{lem:freedman's concetration lemma}) with $R = \frac{3000000\alpha}{C_1}, \sigma^2 = \frac{(3000000\alpha)^2}{C_1}$. We get

\begin{align*}
    \Pr \left(\left|\sum_{i=1}^{k}(Y_i - \E[Y_i | \mathbb{F}_i])\right| \geq \alpha/100 \right) = \Pr \left(\left|\sum_{i=1}^{k'}(Y_i - \E[Y_i | \mathbb{F}_i])\right| \geq \alpha/100 \right) \\
    \leq
    2\exp\left\{-\frac{(\alpha/100)^2/2}{(3000000\alpha)^2/C_1 + \alpha^2 3000000/300C_1}\right\} = 2\exp\left\{-\frac{C_1}{20000(3000000+10000)}\right\} =\\
    2\exp\left\{-\frac{C\log( T \NN(\FF_h,\sqrt{\delta/64T^3})/\delta)}{20000(3000000+10000)}\right\} = 2\exp\left\{-\frac{C(\log(T \NN(\FF_h,\sqrt{\delta/64T^3})/\delta)^2)}{40000(3000000+10000)}\right\} \leq\\
    C' (\delta/64T)^2/ (\NN(\FF_h, \sqrt{\delta/64T^3}))^2
\end{align*}

We can pick $C$ so that $C' = 1$. \todo{they get  $\delta$ instead of $\delta^2$, I'm not sure why. Will check it later. For now I assume that $\delta$ is the correct thing to get and proceed with that.} Now we can take a union bound over all the functions in the discretized set and conclude that with probability at least $1-\delta/(64T^2)$ we have that 

\begin{align*}
    \left|\sum_{i=1}^{k}(Y_i - \E[Y_i | \mathbb{F}_i])\right| \leq \alpha/100
\end{align*}

We condition on this event and \todo{write bound on $\hat{Z}_h^k$, explain that $\hat{f}$ is the LSE wrt the whole dataset}. We first show that when this event happens,  we have that $\underbar{$\CC$}_h^k(\alpha) \subseteq \hat{\CC}_h^k(\alpha)$. Consider $f_1 \in \BB_{h,\ZZ_h^k}(\hat{f}, \alpha/100)$. We know that there exist $f_1',\hat{f}' \in \CC(\FF,\sqrt{\delta/(64T^3)}) \times \CC(\FF,\sqrt{\delta/(64T^3)})$ with $||f_1 - f_1'||_{\infty}, ||\hat{f}-\hat{f}'||_{\infty} \leq \sqrt{\delta/64T^3}$. Hence, we get that 

\begin{align*}
    ||f_1' - \hat{f}'||_{\ZZ_h^k}^2 \leq \left(||f_1 - f_1'||_{\ZZ_h^k}  + ||\hat{f} - \hat{f}'||_{\ZZ_h^k} + ||f_1 - \hat{f}||_{\ZZ_h^k}\right)^2 \\ 
    \leq \left(||f_1 - f_1'||_{\ZZ_h^k}  + 2\sqrt{64\delta|\ZZ_h^k|T^3}\right)^2 \leq  \left(||f_1 - f_1'||_{\ZZ_h^k}  + \frac{2}{T}\sqrt{64\delta}\right)^2 \leq \alpha/50
\end{align*}

We now consider the $Y_i$'s that are generated by $f_1', \hat{f}'$. It holds that $||f_1' - \hat{f}'||^2_{\ZZ_h^k} \leq \alpha/25 \implies ||f_1' - \hat{f}'||^2_{\ZZ_h^{k-1}} \leq \alpha/25$. Since the event $\EE_h^{k-1}$ happens it follows that $\{||f_1' - \hat{f}'||_{\hat{\ZZ}_h^{k-1}}^2,T(H+1)^2 \} \leq 100(\alpha/25) = 4\alpha < 2000000\alpha \implies Z_k \leq 2000000\alpha$. Thus, every $Y_i$ is exactly $(f_1'(z_h^i) - \hat{f}'(z_h^i))^2$ multiplied by the number of times $z_h^i$ is in the sub-sampled dataset. Hence, we get

\begin{align*}
    ||f_1' - \hat{f}'||^2_{\hat{\ZZ}_h^k} = \sum_{i=2}^k Y_i \leq \sum_{i=2}^k\E[Y_i | \mathbb{F}_i] + \alpha/100 \leq ||f'_1 - \hat{f}'||_{\ZZ_h^k}^2 + \alpha/100 \leq 3\alpha/100 
\end{align*}

where the first inequality follows from the concentration bound we have derived and the other two simply from the definitions of these quantities.  

We now bound $||f_1 - \hat{f}||^2_{\hat{\ZZ}_h^k}$. We have that

\begin{align*}
    ||f_1 - \hat{f}||_{\hat{\ZZ}_h^k}^2 \leq (||f_1' - \hat{f}'||_{\hat{\ZZ}_h^k} + ||f_1 - f_1'||_{\hat{\ZZ}_h^k} + ||\hat{f} - \hat{f}'||_{\hat{\ZZ}_h^k})^2 \leq \\
    (||f_1' - \hat{f}'||_{\hat{\ZZ}_h^k} + 2\sqrt{|\hat{\ZZ}_h^k}| \cdot \sqrt{\delta/(64T^3)})^2 \leq (||f_1' - \hat{f}'||_{\hat{\ZZ}_h^k} + 2)^2 \leq (\sqrt{3\alpha/100}+2)^2 \leq \alpha
\end{align*}

Hence, we have shown that $\underbar{$\CC$}_h^k(\alpha) \subseteq \hat{\CC}_h^k(\alpha)$. So in this case, the one inequality that define $\EE_h^k$ holds.\\

We shift our attention to the second inequality now. We will show the contrapositive of our claim, i.e. if $f \notin \overline{C}_h^k(\alpha) \implies f \notin \hat{C}_h^k(\alpha)$. Let $f_1 \in \FF_h$ such that $L_{\ZZ_h^k}(f_1, \hat{f}_h^k) > 100\alpha$.  We know that there exist $f_1',\hat{f}' \in \CC(\FF,\sqrt{\delta/(64T^3)}) \times \CC(\FF,\sqrt{\delta/(64T^3)})$ with $||f_1 - f_1'||_{\infty}, ||\hat{f}-\hat{f}'||_{\infty} \leq \sqrt{\delta/64T^3}$. Hence, using the triangle inequality we get that 

\begin{align*}
    ||f_1' - \hat{f}'||_{\ZZ_h^k}^2 \geq (||f_1-\hat{f}||_{\ZZ_h^k} - ||f_1-f_1'||_{\ZZ_h^k} - ||f_2-f_2'||_{\ZZ_h^k})^2 \geq \\
    (||f_1-\hat{f}||_{\ZZ_h^k} - 2 \sqrt{|\ZZ_h^k|}\sqrt{\delta/(64T^3)})^2 = (\sqrt{100\alpha} - 2 \sqrt{\delta/(64T^2)})^2 > 50\alpha
\end{align*}

Again, consider the $Y_i$'s that are generated by $f_1', \hat{f}'$. We want to show that $||f_1' - \hat{f}'||_{\hat{\ZZ}_h^k}^2 > 40\alpha$. Assume towards contradiction that $||f_1' - \hat{f}'||_{\hat{\ZZ}_h^k}^2 \leq 40\alpha$. We consider three different cases. 

\textbf{First Case: $||f_1' - \hat{f}'||^2_{\ZZ_h^k} \leq 2000000\alpha$}. Similarly as before, we have that

\begin{align*}
    ||f_1' - \hat{f}'||_{\hat{\ZZ}_h^k}^2 = \sum_{i=2}^k Y_i \geq  \sum_{i=2}^k Y_i = \E[Y_i| \mathbb{F}_i] - \alpha/100 > 50\alpha - \alpha/100 > 40\alpha
\end{align*}

So we get a contradiction.

\textbf{Second Case: $||f_1' - \hat{f}'||^2_{\ZZ_h^{k-1}} > 10000\alpha$}. The contradiction comes directly from the fact that $\EE_h^{k-1}$ holds, so $$||f_1' - \hat{f}'||_{\hat{\ZZ}_h^k}^2 \geq ||f_1' - \hat{f}'||_{\hat{\ZZ}_h^{k-1}}^2 > 100\alpha$$


\textbf{Third Case: $||f_1' - \hat{f}'||^2_{\ZZ_h^{k-1}} \leq 10000\alpha$ and $||f_1' - \hat{f}'||^2_{\ZZ_h^k} > 2000000\alpha$}. We can directly see that our assumption and from \todo{add Lemma 3 of previous paper, check if we can make the constant in the probability 1 to make our lives easier} for this case gives us that $(f_1'(z_h^k) - \hat{f}'(z_h^k))^2 \geq 1900000\alpha$. 
Since $||f_1' - \hat{f}'||^2_{\ZZ_h^{k-1}} \leq 10000\alpha \implies ||f_1' - \hat{f}'||^2_{\hat{\ZZ}_h^{k-1}} \leq 1000000\alpha $. 
Thus, since $\alpha \geq \beta$ we can see that the sensitivity is 1 so the element will be added to the sub-sampled dataset.
Hence, $||f_1' - \hat{f}'||_{\ZZ_h^k}^2 \geq (f_1'(z_h^k) - \hat{f}'(z_h^k))^2 > 40\alpha$.

Thus, in any case we have that $||f_1' - \hat{f}'||_{\hat{\ZZ}_h^k}^2 > 40\alpha > \alpha$, so we get the result.


\end{proof}



\begin{prevproof}{Lemma}{lem: mixture mdp: sub-sampled dataset is good approximation to original one}

Now that we have Lemma~\ref{lem:helper lemma to prove approximation of sub-sampled dataset} the proof is exactly the same as in \cite{kong2021online}. I will modify the constants accordingly when we have figured out all the details.

\end{prevproof}

Now that we have proven Lemma~\ref{lem: mixture mdp: sub-sampled dataset is good approximation to original one} here's how we get the regret guarantee based on everything we have proven so far. We have shown with this lemma that $\underline{b}_h^k(\cdot, \cdot) \leq b_h^k(\cdot) \leq \overline{b}_h^k(\cdot, \cdot)$. We also have that $\underbar{$\CC$}_h^k \subseteq \hat{\CC}_h^k(\alpha) \subseteq \overline{\CC}_h^k(\alpha)$. The lower bound of this inequality combined with the arguments of the previous section show that the true function $f^*$ is in our class with high probability at every time step. This is Corollary 17. Notice that if we don't subsample the dataset then Lemma 16 holds. Also, the LSE is the same for all three processes. Then, the proof of Lemma 18 for the sub-sampled dataset is the same. Finally, we can use the bound of Lemma 19 for $\overline{b}_h^k(\cdot, \cdot)$ which will also give us an upper bound on the bonus our algorithm uses. Now everything in the previous section follows. Essentially, we plugin these three results that I mentioned to the next 4 lemmas/theorems.

\todo{Now it only remains to bound the sum of the sensitivities. This should be exactly the same as in their paper. Will do that soon.} 

\begin{lemma}\label{lem:linear mixture mdp-bound on summation of sensitivity}
With probability at least $1-\delta??$ for any fixed $h \in [H]$ we have that the sub-sampled dataset $\hat{Z}_h^k, k \in [K]$ changes at most $$S_{\max} = ??$$ times.
\end{lemma}

We first need the following before we prove this lemma. First, we show that if the dataset is not sub-sampled then the sensitivity scores can be bounded.

\begin{lemma}\label{lem:linear mixture mdp-bound on summation of sensitivity of original set}\cite{kong2021online}
We can bound the summation of the sensitivity parameters as follows. For every $h \in [H]$ we have that 

$$\sum_{k=1}^{K-1} \text{sensitivity}_{\ZZ_h^k, \FF_h}(z_h^k) \leq C \cdot \text{dim}_E(\FF, 1/T) \log((H+1)^2T)\log T$$

where $C > 0$, is some absolute constant.
\end{lemma}

\begin{proof}
The proof is exactly the same as in the original paper (Lemma~5\cite{kong2021online}).
\end{proof}


We are now ready to prove Lemma~\ref{lem:linear mixture mdp-bound on summation of sensitivity}

\begin{prevproof}{Lemma}{lem:linear mixture mdp-bound on summation of sensitivity}
% Throughout the proof, we condition on the event $\E_h^k$ which essentially shows that $\hat{\Z}_h^k$ is a good approximation to $\Z_h^k$. We also fix some $h \in [H]$. Under this event, we have that

% \begin{align*}
%     \text{sensitivity}_{\hat{\ZZ}^k_h,\FF_h}(z_h^k) \leq C\cdot \text{sensitivity}_{\ZZ^k_h,\FF_h}(z_h^k)
% \end{align*}

% for every $k \in [K]$ and some constant $C > 0$. From the definition of $p_z$, we can see that
Actually the proof is again the same as in the original paper.
\end{prevproof}


\todo{Do we need a lower bound of some sort for adaptivity?}

==> lower_bound_adaptivity_bandits.tex <==
\section{Lower Bound for Adaptivity in Stochastic Multi-Armed Bandits}

We follow the approach of~\cite{gao2019batched}.
Let $M$ be the number of policy switches the learner is allowed to make.
We define the \emph{adaptive grid} $\mathcal{T} = \{t_1,\ldots,t_M\}, 1\leq t_1 \leq
\ldots \leq t_M \leq 1$ in the following way: for every $j \in [M]$ the policy of
the learner between $t_j, t_{j+1}$ must depend only on observations prior to $t_j$
and must be fixed.

We first state some results from their paper.

\begin{lemma}
\cite{gao2019batched}
\label{lem:bandits lower bound, helper lemma}
Let $T = (V,E)$ be a tree on $V = [n]$, and $x \in \R^n$ be any vector. Then,
$$\sum_{i=1}^n x_i - \max_{i \in [n]} x_i \geq \sum_{(i,j)\in E}\min\{x_i, x_j\}.$$
\end{lemma}


\begin{lemma}\label{lem:bandits lower bound, helper lemma 2}
\cite{gao2019batched}
Let $Q_1,\ldots,Q_n$ be probability measures and $\Psi: \Omega \rightarrow [n]$
be any measurable function. Then for any tree $T = ([n],E)$ with vertex set
$[n]$ and edge set $E$, we have

\begin{align*}
    \frac{1}{n} \sum_{i=1}^n Q_i(\Psi \neq i) \geq \sum_{(i,j) \in E} \int \min\{dQ_i, dQ_j \},
\end{align*}
\end{lemma}

\begin{lemma}
\cite{gao2019batched}
\label{lem:bandits lower bound, helper lemma 3}
Let $P, Q$ be any probability distributions on the same probability space. Then,

\begin{align*}
    \text{TV}(P,Q) \leq \sqrt{1 - \exp(-D_{\text{KL}}(P||Q))} \leq 1 - \frac{1}{2}\exp(-D_{\text{KL}}(P||Q))
\end{align*}
\end{lemma}

Let $A$ be the number of arms and $T$ the time horizon.
We follow their approach, and for every $j \in [M]$, we define
$$T_j = \lfloor T^{\frac{1-2^{-j}}{1-2^{-M}}} \rfloor, ~~~~\Delta_j = \frac{\sqrt{A}}{36M} T^{\frac{1-2^{1-j}}{1-2^{-M}}}.$$

Moreover, we define a family of reward distributions for every $ a \in [A], j \in [M-1]$:

$$P_{a,j} = \NN(0,1) \times \ldots \times \NN(0,1) \times \NN(\Delta_j + \Delta_M, 1) \times \NN(0,1) \times \NN(0,1) \times \NN(\Delta_M,1)$$

where the $a$-th component of $P_{a,j}$ has non-zero mean. When $j=M$, we define

$$P_M = \NN(0,1) \times \ldots \times \NN(0,1)  \times \NN(\Delta_M,1).$$
We define the event $A_j = \{t_{j-1} < T_{j-1}, t_j \geq T_j \}$. 
Note that these events form a partition of the space. We also denote
$P_{a,i}(A_j)$ be the probability that the event $A_j$ happens when the true
distribution is $P_{a,i}$, the policy is $\pi$ and the learner has seen
the rewards up to time $T_{i-1}$.
\todo{this is slightly different, I think we need to count the probability up to time $T_{j-1}$. this is because the decision to change the policy can be triggered by a reward
that we see in the batch, unlike their setting.}
We also let

$$p_j = \frac{1}{A-1}\sum_{a=1}^{A-1} P_{a,j}(A_j), ~~~~j \in [M-1], ~~~~p_M = P_M(A_M)$$

The next lemma follows the approach of \cite{gao2019batched}.

\begin{lemma}
\label{lem:bandits lower bound, regret is low given some condition}
If $p_j \geq \frac{1}{2M}$ for some $j \in [M]$, then we have that

$$\sup \E[\reg(T)] \geq c M^{-2} \sqrt{A} T^{\frac{1}{1-2^{1-M}}},$$

where $c > 0$ is some absolute constant.
\end{lemma}

\begin{proof}
We prove the lemma when $j \in [M-1]$. The other case follows similarly.
For any $a \in [A]$, we consider the family $\PP_{a, j} = (Q_{a,j,\ell})_{\ell \in [A]}$
of reward distributions, where $Q_{a, j, a} = P_{a,j}$ and for $\ell \neq a$ we
define it to be a perturbed version $P_{j,a}$ where we add the quantity $3\Delta_j$
to the mean of the $\ell$-th component. Observe that
\begin{itemize}
    \item For each $\ell \in [A]$ the optimal arm under $Q_{a,j,\ell}$ is the $\ell$-th.
    \item For each $\ell \in [A]$, pulling some arm $\ell' \neq \ell$
    incurs regret at least $\Delta_j$ under the distribution $Q_{a,j,\ell}$.
    \item For every $\ell \neq a$ the distributions $Q_{a,j,\ell}, Q_{a,j,a}$ differ
    only in the $\ell$-th component.
\end{itemize}

Now we can use the fact that the supremum over the choices of the gaps and the distributions
of the rewards of the arms is bounded below by the average of the distributions we
just defined. Hence, we get

\begin{align*}
    \sup \E[\reg(T)] \geq \Delta_j \sum_{t=1}^T \frac{1}{A}\sum_{\ell = 1}^A Q^t_{a,j,\ell}(\pi_{t} \neq \ell)
\end{align*}

where $Q^t_{a,j,\ell}$ denotes the distribution of the observations available
at time $t$ to the learner to make the decision about the policy. 
Consider a star graph on $[A]$ centered at $a$.
Using Lemma~\ref{lem:bandits lower bound, helper lemma} and 
Lemma~\ref{lem:bandits lower bound, helper lemma 2}, we get

\begin{align*}
    \Delta_j \sum_{t=1}^T \frac{1}{A}\sum_{\ell = 1} Q^t_{a,j,\ell}(\pi_{t} \neq \ell) &\geq
    \Delta_j \sum_{t=1}^T \frac{1}{A}\sum_{\ell \neq a} \int \min\{dQ^t_{a,j,a}, dQ^t_{a,j,\ell}\}\\
    &\geq \Delta_j \sum_{t=1}^{T_j} \frac{1}{A}\sum_{\ell \neq a} \int \min\{dQ^t_{a,j,a}, dQ^t_{a,j,\ell}\}
\end{align*}

where the second inequality is trivial. Now using the fact that $\int\min\{P,Q\} = 1 - TV(P,Q)$
and the data processing inequality, we get that 

\begin{align*}
    \Delta_j \sum_{t=1}^{T_j} \frac{1}{A}\sum_{\ell \neq a} \int \min\{dQ^{t}_{a,j,a}, dQ^{t}_{a,j,\ell}\} &\geq  \Delta_j T_j \frac{1}{A}\sum_{\ell \neq a} \int \min\{dQ^{T_j}_{a,j,a}, dQ^{T_j}_{a,j,\ell}\}\\
    &\geq \Delta_j T_j \frac{1}{A}\sum_{\ell \neq a} \int_{A_j} \min\{dQ^{T_j}_{a,j,a}, dQ^{T_j}_{a,j,\ell}\}
\end{align*}

and the second inequality is trivial. Now notice that whenever $A_j$ happens,
the distribution of the observations that are available to the learner to make
a decision at time $T_j$ is the same as the distribution that is available
at time $T_{j-1}$. Hence 

\begin{align*}
    \Delta_j T_j \frac{1}{A}\sum_{\ell \neq a} \int_{A_j} \min\{dQ^{T_j}_{a,j,a}, dQ^{T_j}_{a,j,\ell}\} = \Delta_j T_j \frac{1}{A}\sum_{\ell \neq a} \int_{A_j} \min\{dQ^{T_{j-1}}_{a,j,a}, dQ^{T_{j-1}}_{a,j,\ell}\}.
\end{align*}

We now focus on the last quantity to derive our lower bound. We have that

\begin{align*}
    \int_{A_j} \min\{dQ^{T_{j-1}}_{a,j,a}, dQ^{T_{j-1}}_{a,j,\ell}\} &= \int_{A_j} \frac{dQ^{T_{j-1}}_{a,j,a} + dQ^{T_{j-1}}_{a,j,\ell} - |dQ^{T_{j-1}}_{a,j,a} - dQ^{T_{j-1}}_{a,j,\ell}|}{2} \\
    &= \frac{Q^{T_{j-1}}_{a,j,a}(A_j) + Q^{T_{j-1}}_{a,j,\ell}(A_j)}{2} - \frac{1}{2}
    \int_{A_j}|dQ^{T_{j-1}}_{a,j,a} - dQ^{T_{j-1}}_{a,j,\ell}|\\
    &\geq \left(Q^{T_{j-1}}_{a,j,a}(A_j) - \frac{1}{2} \text{TV}(Q^{T_{j-1}}_{a,j,a}, Q^{T_{j-1}}_{a,j,\ell})\right) - \text{TV}(Q^{T_{j-1}}_{a,j,a}, Q^{T_{j-1}}_{a,j,\ell}) \\
    &= P_{a,j}(A_j) - \frac{3}{2}\text{TV}(Q^{T_{j-1}}_{a,j,a}, Q^{T_{j-1}}_{a,j,\ell})
 \end{align*}
 
 \todo{the difference is that I've defined the probability $P_{a,j}(A_j)$ to measure up to time $T_{j-1}$ whereas the take it to be the probability over all the execution}
 where the inequality follows from $|P(E) - Q(E)| \leq \text{TV}(P,Q)$. Hence,
 we focus our attention to bounding the total variation distance between the two distributions. Using Lemma~\ref{lem:bandits lower bound, helper lemma 3} we get
 
 \begin{align*}
     \frac{1}{A} \sum_{\ell \neq a} \text{TV}(Q^{T_{j-1}}_{a,j,a}, Q^{T_{j-1}}_{a,j,\ell}) &\leq 
     \frac{1}{A} \sum_{\ell \neq a} \sqrt{1 - \exp\left(D_{\text{KL}}(Q^{T_{j-1}}_{a,j,a}|| Q^{T_{j-1}}_{a,j,\ell})\right)}\\
     &= \frac{1}{A} \sum_{\ell \neq a} \sqrt{1 - \exp\left(-\frac{9\Delta_j^2\E_{P_{a,j}}[\tau_{\ell}]}{2} \right)}\\
     &\leq \frac{A-1}{A} \sqrt{1 - \exp\left( \frac{9\Delta_j^2}{2(A-1)} \sum_{\ell \neq a} \E_{P_{a,j}}[\tau_{\ell}]\right)}\\
     &\leq \frac{A-1}{A} \sqrt{1 - \exp\left( \frac{9\Delta_j^2T_{j-1}}{2(A-1)}  \right)} \leq \frac{3}{\sqrt{A}} \sqrt{\Delta_j^2 T_{j-1}} \leq \frac{1}{12M}
 \end{align*}
 
 where the second equality evaluates the KL-divergence with $\tau_{\ell}$ being 
 the number of times we pull arm $\ell$ before time $T_{j-1}$, the third inequality
 follows from concavity, the fourth one from the fact that $\sum_{\ell \neq a}\tau_{\ell} \leq T_{j-1}$ and then it is just algebra. 
 Putting everything together, we get
 
 \begin{align*}
     \sup \E[\reg(T)] \geq \Delta_j T_j \left(\frac{P_{a,j}}{2} - \frac{1}{8M}\right) \geq
     \sqrt{A} T^{\frac{1}{2-2^{1-M}}} \frac{1}{72M}\left(\frac{P_{a,j}}{2} - \frac{1}{8M} \right).
 \end{align*}
 
 By taking the average over $k \in [K-1]$ we get
 
 \begin{align*}
     \sup \E[\reg(T)]  \geq
     \sqrt{A} T^{\frac{1}{2-2^{1-M}}} \frac{1}{72M}\left(\frac{1}{2(A-1)}\sum_{a=1}^{A-1}P_{a,j} - \frac{1}{8M} \right) \geq \frac{1}{576M^2} T^{\frac{1}{2-2^{1-M}}}.
 \end{align*}
 
 


\end{proof}

The next lemma establishes that the condition required in Lemma~\ref{lem:bandits lower bound, regret is low given some condition}
holds.

\begin{lemma}
\label{lem:bandits lower bound, sum of probabilities is large}
It holds that $$\sum_{j=1}^M p_j \geq \frac{1}{2}.$$
\end{lemma}

\begin{proof}
We have that $|P_M(A_j) - P_{a,j}(A_j)| \leq \text{TV}(P_M^{T_{j-1}}, P_{a,j}^{T_{j-1}})$. Similarly as before, we get that

\begin{align*}
    \frac{1}{A-1} \sum_{a=1}^{A-1} \text{TV}(P_M^{T_{j-1}}, P_{a,j}^{T_{j-1}}) &\leq
    \frac{1}{A-1} \sum_{a=1}^{A-1}  \sqrt{1 - \exp(-D_{\text{KL}}(P_M^{T_{j-1}}||P_{a,j}^{T_{j-1}}))}\\
    &= \frac{1}{A-1} \sum_{a=1}^{A-1} \sqrt{1 - \exp\left(- \frac{(\Delta_j + \Delta_M)^2}{2} \E_{P_{M}}[\tau_a]\right)} \\
    &\leq \sqrt{1- \exp\left(- \frac{2\Delta_j^2}{A-1} \E_{P_{M}}\left[\sum_{a=1}^{A-1}\tau_a\right]\right)}\\
    &\leq \sqrt{1 - \exp\left(- \frac{2\Delta_j^2T_{j-1}}{A-1} \right)} \leq \frac{
    1}{2M}
\end{align*}
where $\tau_a$ is the number of times we pull arm $a$ before time $T_{j-1}$.
Thus, we see that

\begin{align*}
    |P_M(A_j) - p_j| \leq \frac{1}{A-1} \sum_{a=1}^{A-1} |P_M(A_j) - P_{a,j}(A_j)| \leq \frac{1}{2M}.
\end{align*}

Moreover, by summing up over $j$ we get

\begin{align*}
    \sum_{j=1}^M p_j \geq P_M(A_m) + \sum_{j=1}^{M-1} \left(P_M(A_j) - \frac{1}{2M}\right) \geq \sum_{j=1}^{M}P_M(A_j) - \frac{1}{2}
\end{align*}

The proof follows by taking a union bound and recalling that $A_1, \ldots, A_M$
partition the space.
\end{proof}



